ROSA: Random Subspace Adaptation for Efficient Fine-Tuning

Model training requires significantly more memory, compared with inference. Parameter efficient fine-tuning (PEFT) methods provide a means of adapting large models to downstream tasks using less memory. However, existing methods such as adapters, prompt tuning or low-rank adaptation (LoRA) either introduce latency overhead at inference time or achieve subpar downstream performance compared with full fine-tuning. In this work we propose Random Subspace Adaptation (ROSA), a method that outperforms previous PEFT methods by a significant margin, while maintaining a zero latency overhead during inference time. In contrast to previous methods, ROSA is able to adapt subspaces of arbitrarily large dimension, better approximating full-finetuning. We demonstrate both theoretically and experimentally that this makes ROSA strictly more expressive than LoRA, without consuming additional memory during runtime. As PEFT methods are especially useful in the natural language processing domain, where models operate on scales that make full fine-tuning very expensive, we evaluate ROSA in two common NLP scenarios: natural language generation (NLG) and natural language understanding (NLU) with GPT-2 and RoBERTa, respectively. We show that on almost every GLUE task ROSA outperforms LoRA by a significant margin, while also outperforming LoRA on NLG tasks. Our code is available at https://github.com/rosa-paper/rosa

==> figures/crown_jewel.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
  arrowHead/.style={-{Triangle[width=2mm, length=2mm]}},
  arrowLine/.style={line width=1mm},
  arrowLineDashed/.style={line width=1mm, dashed, dash pattern=on 3mm off 2mm},
  square/.style={draw, rectangle, rounded corners=1mm, minimum width=2cm, minimum height=1.75cm, fill=blue!20, font=\small},
  trapezium/.style={draw, shape=trapezium, trapezium left angle=70, trapezium right angle=70, minimum width=2cm, minimum height=0.75cm, rounded corners=1mm, fill=green!20, font=\small},
  rectangle/.style={draw, rounded corners=1mm, minimum width=5cm, minimum height=0.75cm, fill=red!20, font=\small}
]

    \node[rectangle] (rectangle1) at (0, 2cm) {$\vec{h}$};
    
    \node[square ] (square) at (-2.6cm, 0) {$\mat{w}_{\text{f}} \gets \mat{U}_{R^{\prime}} \mat{\Sigma}_{R^{\prime}} \mat{V}^\top_{R^{\prime}} $};

    \draw[arrowHead, arrowLineDashed] (45:1cm) arc[start angle=45, end angle=135, radius=1cm];
    \draw[arrowHead, arrowLineDashed] (225:1cm) arc[start angle=225, end angle=315, radius=1cm];
    
    \node[font=\tiny] at (0,0) {\parbox{2.5cm}{\centering Factorize \\ $\mat{W} = \mat{W}_\text{f} + \mat{A}\mat{B}$}};

    \node[trapezium] (top_trap) at (2.6cm, 0.5) {$\mat{b} \gets \mat{\Sigma}^{\frac{1}{2}}_{R^{\prime\prime}} \mat{V}^\top_{R^{\prime\prime}}$};
    \node[trapezium, shape border rotate=180] (bottom_trap) at (2.6cm, -0.5) {$\mat{a} \gets \mat{U}_{R^{\prime\prime}} \mat{\Sigma}^{\frac{1}{2}}_{R^{\prime\prime}} $};

    \node[rectangle] (rectangle2) at (0, -2cm) {$\vec{x}$};

    % Empty
    \node[minimum height=0.75cm] (e1_target) at ([shift={(-1.5cm,-0.1cm)}]rectangle1.south) {};
    \node[minimum height=0.75cm] (e1_source) at ([shift={(0,0.1cm)}]square.north) {};

    \node[minimum height=0.75cm] (e2_target) at ([shift={(1.5cm,-0.1cm)}]rectangle1.south) {};
    \node[minimum height=0.75cm] (e2_source) at ([shift={(0,0.1cm)}]top_trap.north) {};

    \node[minimum height=0.75cm] (e3_source) at ([shift={(-1.5cm, 0.1cm)}]rectangle2.north) {};
    \node[minimum height=0.75cm] (e3_target) at ([shift={(0,-0.1cm)}]square.south) {};

    \node[minimum height=0.75cm] (e4_source) at ([shift={(1.5cm, 0.1cm)}]rectangle2.north) {};
    \node[minimum height=0.75cm] (e4_target) at ([shift={(0,-0.1cm)}]bottom_trap.south) {};

    \draw[arrowHead, arrowLine] (e1_source) -- (e1_target);
    \draw[arrowHead, arrowLine] (e2_source) -- (e2_target);
    \draw[arrowHead, arrowLine] (e3_source) -- (e3_target);
    \draw[arrowHead, arrowLine] (e4_source) -- (e4_target);
    
\end{tikzpicture}

\caption{Illustration of ROSA. Parameter matrix $\mat{W}$ is factorized using SVD and split into smaller trainable matrices $(\mat{A}, \mat{B})$ and a larger fixed matrix $(\mat{W}_{\text{f}})$. The split is then merged after a specified number of training iterations, and the process is repeated. ROSA updates an increasingly larger subspace of $\mat{W}$ over the course of training while remaining memory efficient}
\label{fig:crown-jewel}
\end{figure}
